Stability Analysis of Planar Probabilistic Piecewise Constant Derivative Systems

In this paper, we study the probabilistic stability analysis of a subclass of stochastic hybrid systems, called the Planar Probabilistic Piecewise Constant Derivative Systems (Planar PPCD), where the continuous dynamics is deterministic, constant rate and planar, the discrete switching between the modes is probabilistic and happens at boundary of the invariant regions, and the continuous states are not reset during switching. These aptly model piecewise linear behaviors of planar robots. Our main result is an exact algorithm for deciding absolute and almost sure stability of Planar PPCD under some mild assumptions on mutual reachability between the states and the presence of non-zero probability self-loops. Our main idea is to reduce the stability problems on planar PPCD into corresponding problems on Discrete Time Markov Chains with edge weights.

==> exp.tex <==
\section{Experiments and Observations}

\input{table}

For experiment, we convert 2D PPCD into its quotient WDTMC and apply Algorithm 
\ref{alg_abs_conv} (Algorithm \ref{alg_as_conv}) on the quotient WDTMC to decide whether it is 
absolutely (almost surely) stable.
The entire procedure has been implemented in a Python toolbox.
We represent the PPCD and the quotient WDTMC as annotated graphs and
use \emph{networkx}  \cite{SciPyProceedings_11} module of Python to
store and manipulate these entities.
To calculate the edge weights, we need to solve linear optimization problem (as discussed in 
\cite{prabhakar2013abstraction}) and that is done by \emph{pplpy}, a Python module for Parma 
Polyhedra Library (PPL) \cite{Bagnara2008}. We use \emph{networkx} 
\cite{SciPyProceedings_11} functions to find the existence of infinite
weighted edges and simple cycles with weight greater than or equal to $0$, to check
for absolute stability of the PPCD.
To compute almost sure stability, we need to calculate the stationary
distribution of the quotient WDTMC, which requires solving a set of
linear equations mentioned in Definition \ref{stn_dist}.
We use pplpy \cite{Bagnara2008} for solving the feasibility of linear
equations.
Our experiments have been performed on macOS Big Sur with Quad-Core
Intel Core i7 2.8GHz$\times$ 1 Processor and 16GB RAM. 

We have analyzed six examples of PPCD with various number of locations.
In the first three examples, we partitioned the $XY$ plane into $4$ regions (one region corresponding 
to each quadrant) and assigned $6$ locations to each region (thus, total $6\times4=24$ locations).
In the other three examples, we partitioned the $XY$ plane into $8$
regions, corresponding to splitting each of the quadrants diagonally
into two, and assigned $12$ locations to each region (thus, total $12\times 8=96$ locations).
The  guard for all locations corresponding to a region is set to the facet of that region that 
makes a larger angle with positive $X$-axis. The Flow for each location is of the form 
$a\dot{x}+b\dot{y}=0$, where $a$ and $b$ 
depend on the corresponding region and experiment. For example, in the first experiment, for region 
$1$, $a=1$ and $b$ is randomly chosen between $\{1,\dots,5\}$, for region
$2$, $b=1$ and $-a$ is randomly chosen between $\{1,\dots,5\}$, for region 
$3$, $a=-1$ and $-b$ is randomly chosen between $\{1,\dots,5\}$, and finally, for region 
$4$, $b=-1$ and $a$ is randomly chosen between $\{1,\dots,5\}$. In the second experiment, 
same is done except for the locations corresponding to first region, where we have chosen $a=100$  
so that the PPCD 
will not be absolutely stable. 
For the third experiment also, we have only changed flow for the first 
location with $a=1$ and $b=-4$, so that the PPCD has an infinite edge. 
The fourth experiment was designed similar to the first one. 
For regions 
$1$ and $2$, $a=1$ and $b$ is randomly chosen between $\{1,\dots,5\}$, for region
$3$ and $4$, $b=1$ and $-a$ is randomly chosen between $\{1,\dots,5\}$, for region 
$5$ and $6$, $a=-1$ and $-b$ is randomly chosen between $\{1,\dots,5\}$, and finally, for region 
$7$ and $8$, $b=-1$ and $a$ is randomly chosen between $\{1,\dots,5\}$. 
The fifth and sixth experiments were same as the fourth, except the flow for the first locations were 
modified such that the PPCD in the fifth experiment is not absolutely stable and the PPCD in the 
sixth experiment has an infinite edge, respectively.
The probabilities for change of 
locations are chosen randomly. Note that, all linear equations have integer coefficients and all 
probabilities are rational since PPL cannot handle linear equations with real coefficients.

We present our observations in Table \ref{expt_table}. Here $N$ represents the experiment number, 
$Locs$ represents the number of locations in the PPCD, $\textit{Abs Stability}$ denotes absolute 
stability, $\textit{AS Stability}$ 
denotes almost sure stability, $T_{\textit{conv}}$ is
the processor time to construct the quotient WDTMC, $T_{\textit{abs}}$ is the
processor time required to check absolute stability and $T_{\textit{as}}$ is the processor time required 
to 
check almost sure stability on the reduced system.
In all the three cases, the experimental result 
agreed with the expected result. Note that computing the quotient WDTMC is the most expensive part 
of the analysis, since it requires solving linear optimization problems proportional to $\size{\loc}^2$, 
where $\loc$ is the set of locations of the PPCD. Analyses of both absolute and almost sure stability are 
fast compared to the quotient construction time, however, checking almost sure stability takes 
relatively longer since it requires the computation of the stationary distribution.

==> table.tex <==
\begin{table}
	\resizebox{\textwidth}{!}{%
		\begin{tabular}{|c|c|cc|ccc|}
			\hline
			\multicolumn{1}{|l|}{} & \multicolumn{1}{l|}{} & \multicolumn{2}{c|}{Status}    & 
			\multicolumn{3}{c|}{Time (sec)}                                  \\ \hline
			N & Locs & \multicolumn{1}{c|}{Abs Stability} & AS Stability & 
			\multicolumn{1}{c|}{$T_{\textit{conv}}$} & \multicolumn{1}{c|}{$T_{\textit{abs}}$} & 
			$T_{\textit{as}}$ \\ \hline
			1                      & 24                    & \multicolumn{1}{c|}{Yes} & Yes & \multicolumn{1}{c|}{2.282}  
			& \multicolumn{1}{c|}{0.004} & 0.006 \\ \hline
			2                      & 24                    & \multicolumn{1}{c|}{No}  & No  & \multicolumn{1}{c|}{2.184}  
			& \multicolumn{1}{c|}{0.004} & 0.006 \\ \hline
			3                      & 24                    & \multicolumn{1}{c|}{No}  & No  & \multicolumn{1}{c|}{2.201}  
			& \multicolumn{1}{c|}{0.002} & 0.002 \\ \hline
			4                      & 96                    & \multicolumn{1}{c|}{No}  & Yes & \multicolumn{1}{c|}{24.135} 
			& \multicolumn{1}{c|}{0.066} & 0.091 \\ \hline
			5                      & 96                    & \multicolumn{1}{c|}{No}  & Yes & 
			\multicolumn{1}{c|}{24.626} & \multicolumn{1}{c|}{0.071} & 0.089 \\ \hline
			6                      & 96                    & \multicolumn{1}{c|}{No}  & No  & \multicolumn{1}{c|}{24.477} 
			& \multicolumn{1}{c|}{0.009} & 0.009 \\ \hline
		\end{tabular}%
	}
\caption{Experimental Verification of Stability of Planar $\ppcd$}
\label{expt_table}
\end{table}
